MurTree: Optimal Classification Trees via Dynamic Programming and Search

Decision tree learning is a widely used approach in machine learning, favoured in applications that require concise and interpretable models. Heuristic methods are traditionally used to quickly produce models with reasonably high accuracy. A commonly criticised point, however, is that the resulting trees may not necessarily be the best representation of the data in terms of accuracy and size. In recent years, this motivated the development of optimal classification tree algorithms that globally optimise the decision tree in contrast to heuristic methods that perform a sequence of locally optimal decisions. We follow this line of work and provide a novel algorithm for learning optimal classification trees based on dynamic programming and search. Our algorithm supports constraints on the depth of the tree and number of nodes. The success of our approach is attributed to a series of specialised techniques that exploit properties unique to classification trees. Whereas algorithms for optimal classification trees have traditionally been plagued by high runtimes and limited scalability, we show in a detailed experimental study that our approach uses only a fraction of the time required by the state-of-the-art and can handle datasets with tens of thousands of instances, providing several orders of magnitude improvements and notably contributing towards the practical realisation of optimal decision trees.

==> out_of_sample.tex <==
\begin{table}[t]
\caption{(Upper half of the table) Comparison of our optimal classification trees and conventional heuristic approaches, CART and random forests. For each dataset, the number of instances, number of binary features, and number of classes are displayed. Training and testing accuracies using five-fold cross validation. Each method evaluated on exactly the same folds. Depth and size of the best trees given. Time is the total time to evaluate and train. Legend: MT-F, MT-R, and MT-A are our approach using fixed parameter based on CART, r parameter options based on CART, all parameter settings.\label{table:outofsample}}%
\centering
\def\d{@{\hspace*{1.7mm}}}
\resizebox{\columnwidth}{!}{
\begin{tabular}{ \d l | c | c | c | c | c | c | c | c | c | c | c | c | c | c | c | c | c | c | c | c | c | c | c | c | c \d }

	 &  &  &  & \multicolumn{3}{|c}{Random Forest} & \multicolumn{4}{|c}{CART} & \multicolumn{5}{|c}{MT-F} & \multicolumn{5}{|c}{MT-R}  & \multicolumn{5}{|c}{MT-A}   \\ 
	Name &  $|\mathcal{D}|$ & $|\mathcal{F}|$ & $|\mathcal{C}|$ &  train &  test & time &  train &  test &  d &  s &  train &  test &  d &  s &  time &  train &  test &  d &  s &  time &  train &  test &  d &  s &  time \\ \hline
	anneal & 812 & 93 & 2 & 0.86 & 0.84 & 24 & 0.82 & 0.81 & 3 & 6 & 0.85 & 0.84 & 3 & 6 & $<0.5$& 0.85 & 0.84 & 3 & 4 & $<0.5$& 0.89 & \textbf{0.87} & 4 & 12 & 9 \\ 
	audiology & 216 & 148 & 2 & 0.91 & 0.89 & 18 & 0.94 & 0.92 & 2 & 2 & 0.95 & 0.95 & 2 & 2 & $<0.5$& 0.95 & 0.95 & 2 & 2 & $<0.5$& 0.95 & \textbf{0.95} & 2 & 2 & 9 \\ 
	australian-credit & 653 & 125 & 2 & 0.89 & 0.85 & 23 & 0.87 & 0.85 & 1 & 1 & 0.86 & 0.86 & 1 & 1 & $<0.5$& 0.86 & 0.86 & 1 & 1 & $<0.5$& 0.89 & \textbf{0.87} & 4 & 5 & 36 \\ 
	breast-wisconsin & 683 & 120 & 2 & 0.97 & 0.96 & 22 & 0.96 & 0.93 & 4 & 13 & 0.99 & 0.95 & 4 & 13 & 1 & 0.98 & 0.97 & 3 & 4 & 16 & 0.98 & \textbf{0.97} & 3 & 4 & 16 \\ 
	diabetes & 768 & 112 & 2 & 0.82 & 0.75 & 24 & 0.76 & 0.74 & 3 & 7 & 0.79 & 0.74 & 3 & 7 & $<0.5$& 0.77 & 0.77 & 2 & 2 & $<0.5$& 0.77 & \textbf{0.77} & 2 & 2 & 38 \\ 
	german-credit & 1000 & 112 & 2 & 0.8 & 0.72 & 27 & 0.73 & 0.71 & 3 & 7 & 0.77 & 0.73 & 3 & 7 & $<0.5$& 0.75 & 0.73 & 3 & 4 & 1 & 0.75 & \textbf{0.73} & 3 & 4 & 44 \\ 
	heart-cleveland & 296 & 95 & 2 & 0.89 & 0.79 & 16 & 0.82 & 0.75 & 3 & 7 & 0.87 & 0.74 & 3 & 7 & $<0.5$& 0.83 & 0.77 & 3 & 3 & $<0.5$& 0.93 & \textbf{0.79} & 4 & 14 & 12 \\ 
	hepatitis & 137 & 68 & 2 & 0.92 & 0.82 & 15 & 0.89 & 0.8 & 1 & 1 & 0.86 & 0.86 & 1 & 1 & $<0.5$& 0.86 & 0.86 & 1 & 1 & $<0.5$& 0.86 & \textbf{0.86} & 1 & 1 & 2 \\ 
	hypothyroid & 3247 & 88 & 2 & 0.97 & 0.96 & 34 & 0.98 & 0.98 & 4 & 11 & 0.98 & 0.98 & 4 & 11 & 2 & 0.98 & 0.98 & 2 & 2 & 31 & 0.98 & \textbf{0.98} & 2 & 2 & 35 \\ 
	ionosphere & 351 & 445 & 2 & 0.92 & 0.89 & 31 & 0.9 & 0.88 & 2 & 3 & 0.79 & 0.8 & 2 & 3 & $<0.5$& 0.91 & 0.91 & 2 & 2 & $<0.5$& 0.91 & \textbf{0.91} & 2 & 2 & 2701 \\ 
	kr-vs-kp & 3196 & 73 & 2 & 0.9 & 0.89 & 38 & 0.82 & 0.82 & 4 & 7 & 0.95 & 0.95 & 4 & 7 & 2 & 0.95 & 0.95 & 4 & 7 & 16 & 0.95 & \textbf{0.95} & 4 & 7 & 27 \\ 
	letter & 20000 & 224 & 2 & 0.97 & 0.97 & 534 & 0.97 & 0.97 & 4 & 15 & 0.99 & 0.99 & 4 & 15 & 289 & 0.99 & 0.99 & 4 & 6 & 5004 & 0.99 & \textbf{0.99} & 4 & 6 & 5980 \\ 
	lymph & 148 & 68 & 2 & 0.9 & 0.83 & 15 & 0.87 & 0.81 & 2 & 3 & 0.66 & 0.67 & 2 & 3 & $<0.5$& 0.84 & 0.84 & 2 & 2 & $<0.5$& 0.92 & \textbf{0.85} & 3 & 6 & 3 \\ 
	mushroom & 8124 & 119 & 2 & 0.96 & 0.96 & 74 & 0.94 & 0.94 & 4 & 8 & 1 & 1 & 4 & 8 & 2 & 1 & 1 & 3 & 5 & 84 & 1 & \textbf{1} & 3 & 5 & 88 \\ 
	pendigits & 7494 & 216 & 2 & 0.97 & 0.97 & 143 & 0.97 & 0.97 & 4 & 14 & 1 & 1 & 4 & 14 & 69 & 1 & 1 & 4 & 7 & 1589 & 1 & \textbf{1} & 4 & 7 & 1915 \\ 
	primary-tumor & 336 & 31 & 2 & 0.85 & 0.79 & 15 & 0.84 & 0.8 & 2 & 3 & 0.76 & 0.76 & 2 & 3 & $<0.5$& 0.83 & 0.83 & 2 & 2 & $<0.5$& 0.87 & \textbf{0.85} & 3 & 6 & 1 \\ 
	segment & 2310 & 235 & 2 & 0.99 & 0.99 & 39 & 0.99 & 0.99 & 4 & 5 & 1 & 1 & 4 & 5 & 1 & 1 & 1 & 3 & 3 & 71 & 1 & \textbf{1} & 3 & 3 & 75 \\ 
	soybean & 630 & 50 & 2 & 0.91 & 0.89 & 17 & 0.9 & 0.88 & 4 & 10 & 0.98 & 0.96 & 4 & 10 & $<0.5$& 0.96 & 0.96 & 4 & 6 & 2 & 0.96 & \textbf{0.96} & 4 & 6 & 2 \\ 
	splice-1 & 3190 & 287 & 2 & 0.92 & 0.9 & 88 & 0.88 & 0.88 & 4 & 14 & 0.96 & 0.96 & 4 & 14 & 155 & 0.96 & 0.96 & 4 & 9 & 1756 & 0.96 & \textbf{0.96} & 4 & 9 & 2008 \\ 
	tic-tac-toe & 958 & 27 & 2 & 0.8 & 0.79 & 18 & 0.75 & 0.73 & 4 & 13 & 0.87 & 0.79 & 4 & 13 & $<0.5$& 0.86 & 0.82 & 4 & 11 & 2 & 0.86 & \textbf{0.82} & 4 & 11 & 2 \\ 
	vehicle & 846 & 252 & 2 & 0.9 & 0.89 & 30 & 0.89 & 0.87 & 4 & 12 & 0.99 & 0.96 & 4 & 12 & 11 & 0.97 & 0.97 & 3 & 6 & 315 & 0.97 & \textbf{0.97} & 3 & 6 & 317 \\ 
	vote & 435 & 48 & 2 & 0.97 & 0.95 & 15 & 0.97 & 0.95 & 3 & 7 & 0.98 & 0.93 & 3 & 7 & $<0.5$& 0.96 & 0.96 & 1 & 1 & $<0.5$& 0.96 & \textbf{0.96} & 1 & 1 & 2 \\ 
	yeast & 1484 & 89 & 2 & 0.78 & 0.71 & 29 & 0.71 & 0.7 & 4 & 12 & 0.76 & 0.69 & 4 & 12 & 2 & 0.74 & 0.73 & 4 & 5 & 28 & 0.74 & \textbf{0.73} & 4 & 5 & 33 \\ 
	compas-binary & 6907 & 12 & 2 & 0.66 & 0.66 & 38 & 0.65 & 0.65 & 4 & 15 & 0.67 & 0.67 & 4 & 15 & $<0.5$& 0.67 & 0.67 & 3 & 4 & 2 & 0.67 & \textbf{0.67} & 3 & 4 & 2 \\ 
	fico-binary & 10459 & 17 & 2 & 0.73 & 0.7 & 71 & 0.7 & 0.7 & 4 & 15 & 0.72 & 0.71 & 4 & 15 & 1 & 0.72 & 0.72 & 4 & 5 & 8 & 0.72 & \textbf{0.72} & 4 & 5 & 8 \\ 
	balance-scale & 625 & 4 & 3 & 0.76 & 0.72 & 15 & 0.71 & 0.67 & 3 & 7 & 0.76 & 0.71 & 3 & 7 & $<0.5$& 0.76 & 0.71 & 3 & 5 & $<0.5$& 0.76 & \textbf{0.71} & 3 & 5 & $<0.5$\\ 
	banknote & 1372 & 16 & 2 & 0.89 & 0.89 & 17 & 0.84 & 0.84 & 4 & 5 & 0.92 & 0.92 & 4 & 5 & $<0.5$& 0.92 & 0.92 & 4 & 5 & $<0.5$& 0.95 & \textbf{0.95} & 4 & 9 & $<0.5$\\ 
	bank\_conv & 4521 & 26 & 2 & 0.9 & 0.89 & 35 & 0.9 & 0.89 & 2 & 3 & 0.89 & 0.88 & 2 & 3 & $<0.5$& 0.89 & 0.89 & 1 & 1 & $<0.5$& 0.9 & \textbf{0.9} & 3 & 3 & 5 \\ 
	biodeg & 1055 & 81 & 2 & 0.85 & 0.81 & 23 & 0.8 & 0.78 & 4 & 15 & 0.89 & 0.85 & 4 & 15 & 1 & 0.88 & 0.87 & 4 & 10 & 21 & 0.88 & \textbf{0.87} & 4 & 10 & 24 \\ 
	car\_evaluation & 1728 & 7 & 4 & 0.79 & 0.78 & 17 & 0.78 & 0.78 & 4 & 5 & 0.85 & 0.85 & 4 & 5 & $<0.5$& 0.85 & 0.85 & 4 & 4 & $<0.5$& 0.85 & \textbf{0.85} & 4 & 4 & $<0.5$\\ 
	default\_credit & 30000 & 44 & 4 & 0.62 & 0.55 & 283 & 0.52 & 0.52 & 4 & 15 & 0.58 & 0.58 & 4 & 15 & 7 & 0.58 & 0.58 & 4 & 13 & 148 & 0.58 & \textbf{0.58} & 4 & 13 & 156 \\ 
	HTRU\_2 & 17898 & 57 & 2 & 0.97 & 0.96 & 139 & 0.97 & 0.97 & 3 & 7 & 0.98 & 0.98 & 3 & 7 & 2 & 0.98 & 0.98 & 3 & 3 & 2 & 0.98 & \textbf{0.98} & 3 & 3 & 104 \\ 
	IndiansDiabetes & 768 & 11 & 2 & 0.78 & 0.75 & 18 & 0.76 & 0.74 & 1 & 1 & 0.75 & 0.75 & 1 & 1 & $<0.5$& 0.75 & 0.75 & 1 & 1 & $<0.5$& 0.79 & \textbf{0.77} & 4 & 6 & $<0.5$\\ 
	Ionosphere & 351 & 143 & 2 & 0.94 & 0.91 & 21 & 0.91 & 0.89 & 4 & 7 & 0.97 & 0.9 & 4 & 7 & 2 & 0.95 & 0.94 & 4 & 4 & 27 & 0.95 & \textbf{0.94} & 4 & 4 & 34 \\ 
	iris & 150 & 12 & 3 & 0.96 & 0.94 & 14 & 0.89 & 0.88 & 3 & 4 & 0.96 & 0.94 & 2 & 2 & $<0.5$& 0.96 & 0.94 & 2 & 2 & $<0.5$& 0.96 & \textbf{0.94} & 2 & 2 & $<0.5$\\ 
	magic04 & 19020 & 79 & 2 & 0.79 & 0.76 & 232 & 0.77 & 0.77 & 4 & 15 & 0.82 & 0.82 & 4 & 15 & 7 & 0.82 & 0.82 & 4 & 12 & 149 & 0.82 & \textbf{0.82} & 4 & 12 & 155 \\ 
	messidor & 1151 & 24 & 2 & 0.67 & 0.65 & 19 & 0.64 & 0.62 & 3 & 7 & 0.62 & 0.6 & 3 & 7 & $<0.5$& 0.67 & 0.65 & 3 & 4 & $<0.5$& 0.69 & \textbf{0.66} & 4 & 12 & 2 \\ 
	monk1\_bin & 124 & 15 & 2 & 0.88 & 0.81 & 15 & 0.81 & 0.77 & 3 & 4 & 0.91 & 0.91 & 3 & 4 & $<0.5$& 0.91 & 0.91 & 3 & 4 & $<0.5$& 1 & \textbf{1} & 4 & 8 & $<0.5$\\ 
	monk2\_bin & 169 & 15 & 2 & 0.77 & 0.61 & 15 & 0.68 & 0.59 & 1 & 1 & 0.63 & 0.59 & 1 & 1 & $<0.5$& 0.63 & 0.59 & 1 & 1 & $<0.5$& 0.77 & \textbf{0.67} & 3 & 6 & $<0.5$\\ 
	monk3\_bin & 122 & 15 & 2 & 0.94 & 0.91 & 15 & 0.9 & 0.88 & 2 & 3 & 0.78 & 0.78 & 2 & 3 & $<0.5$& 0.93 & 0.93 & 2 & 2 & $<0.5$& 0.93 & \textbf{0.93} & 2 & 2 & $<0.5$\\ 
	seismic\_bumps & 2584 & 10 & 2 & 0.93 & 0.93 & 22 & 0.93 & 0.93 & 1 & 1 & 0.93 & 0.93 & 1 & 1 & $<0.5$& 0.93 & 0.93 & 1 & 1 & $<0.5$& 0.93 & \textbf{0.93} & 1 & 1 & $<0.5$\\ 
	spambase & 4601 & 132 & 2 & 0.9 & 0.88 & 81 & 0.85 & 0.84 & 4 & 14 & 0.92 & 0.91 & 4 & 14 & 8 & 0.91 & 0.91 & 4 & 7 & 172 & 0.91 & \textbf{0.91} & 4 & 7 & 186 \\ 
	Statlog\_satellite & 4435 & 385 & 6 & 0.74 & 0.71 & 194 & 0.55 & 0.54 & 4 & 15 & 0.77 & 0.76 & 4 & 15 & 270 & 0.76 & 0.76 & 4 & 12 & 4839 & 0.76 & \textbf{0.76} & 4 & 12 & 5148 \\ 
	Statlog\_shuttle & 43500 & 181 & 7 & 0.9 & 0.9 & 1273 & 0.93 & 0.93 & 4 & 10 & 1 & 1 & 4 & 10 & 49 & 1 & 1 & 4 & 6 & 2033 & 1 & \textbf{1} & 4 & 6 & 2125 \\ 
	tic-tac-toe\_bin & 958 & 18 & 2 & 0.81 & 0.8 & 17 & 0.75 & 0.73 & 4 & 13 & 0.87 & 0.79 & 4 & 13 & $<0.5$& 0.86 & 0.82 & 4 & 11 & 1 & 0.86 & \textbf{0.82} & 4 & 11 & 1 \\ 
	winequality-red & 1599 & 17 & 6 & 0.62 & 0.58 & 21 & 0.58 & 0.57 & 3 & 7 & 0.6 & 0.57 & 3 & 7 & $<0.5$& 0.58 & 0.58 & 3 & 3 & $<0.5$& 0.62 & \textbf{0.6} & 4 & 11 & 1 \\ 
	wine & 178 & 32 & 3 & 0.98 & 0.96 & 15 & 0.88 & 0.84 & 3 & 4 & 1 & 0.97 & 4 & 6 & $<0.5$& 0.99 & 0.98 & 4 & 5 & $<0.5$& 0.99 & \textbf{0.98} & 4 & 5 & $<0.5$\\ 
\end{tabular}
}
\end{table}


==> out_of_sample2.tex <==
\begin{table}[t]
\caption{(Lower half of the table) Comparison of our optimal classification trees and conventional heuristic approaches, CART and random forests. For each dataset, the number of instances, number of binary features, and number of classes are displayed. Training and testing accuracies using five-fold cross validation. Each method evaluated on exactly the same folds. Depth and size of the best trees given. Time is the total time to evaluate and train. Legend: MT-F, MT-R, and MT-A are our approach using fixed parameter based on CART, r parameter options based on CART, all parameter settings.\label{table:outofsample2}}%
\centering
\def\d{@{\hspace*{1.7mm}}}
\resizebox{\columnwidth}{!}{
\begin{tabular}{ \d l | c | c | c | c | c | c | c | c | c | c | c | c | c | c | c | c | c | c | c | c | c | c | c | c | c \d }

	 &  &  &  & \multicolumn{3}{|c}{Random Forest} & \multicolumn{4}{|c}{CART} & \multicolumn{5}{|c}{MT-F} & \multicolumn{5}{|c}{MT-R}  & \multicolumn{5}{|c}{MT-A}   \\ 
	Name &  $|\mathcal{D}|$ & $|\mathcal{F}|$ & $|\mathcal{C}|$ &  train &  test & time &  train &  test &  d &  s &  train &  test &  d &  s &  time &  train &  test &  d &  s &  time &  train &  test &  d &  s &  time \\ \hline
	appendicitis-un & 106 & 530 & 2 & 0.86 & 0.8 & 17 & 0.87 & 0.79 & 1 & 1 & 0.84 & 0.8 & 1 & 1 & $<0.5$& 0.84 & 0.8 & 1 & 1 & $<0.5$& 0.86 & \textbf{0.84} & 2 & 2 & 146 \\ 
	australian-un & 690 & 1163 & 2 & 0.82 & 0.77 & 47 & 0.87 & 0.84 & 1 & 1 & 0.86 & 0.86 & 1 & 1 & 1 & 0.86 & 0.86 & 1 & 1 & $<0.5$& 0.86 & \textbf{0.86} & 1 & 1 & 11102 \\ 
	backache-un & 180 & 475 & 2 & 0.9 & 0.86 & 19 & 0.9 & 0.83 & 1 & 1 & 0.88 & 0.82 & 1 & 1 & $<0.5$& 0.88 & 0.82 & 1 & 1 & $<0.5$& 0.86 & \textbf{0.86} & 2 & 3 & 325 \\ 
	cancer-un & 683 & 89 & 2 & 0.96 & 0.94 & 19 & 0.94 & 0.93 & 3 & 6 & 0.98 & 0.93 & 3 & 6 & 1 & 0.97 & 0.94 & 3 & 6 & 7 & 0.97 & \textbf{0.94} & 3 & 6 & 8 \\ 
	car-un & 1728 & 21 & 2 & 0.86 & 0.85 & 22 & 0.83 & 0.83 & 4 & 5 & 0.91 & 0.91 & 4 & 5 & $<0.5$& 0.91 & 0.91 & 4 & 5 & $<0.5$& 0.91 & \textbf{0.91} & 4 & 5 & 2 \\ 
	cleve-un & 303 & 395 & 2 & 0.87 & 0.79 & 18 & 0.83 & 0.79 & 3 & 7 & 0.87 & 0.81 & 3 & 7 & $<0.5$& 0.86 & 0.83 & 3 & 5 & 1 & 0.86 & \textbf{0.83} & 3 & 5 & 182 \\ 
	colic-un & 368 & 415 & 2 & 0.85 & 0.79 & 21 & 0.87 & 0.84 & 2 & 3 & 0.75 & 0.73 & 2 & 3 & $<0.5$& 0.86 & 0.85 & 2 & 2 & $<0.5$& 0.86 & \textbf{0.85} & 2 & 2 & 526 \\ 
	corral-un & 160 & 6 & 2 & 0.93 & 0.91 & 13 & 0.84 & 0.81 & 4 & 11 & 1 & 1 & 4 & 11 & $<0.5$& 1 & 1 & 4 & 7 & $<0.5$& 1 & \textbf{1} & 4 & 7 & $<0.5$\\ 
	haberman-un & 306 & 92 & 2 & 0.8 & 0.73 & 15 & 0.76 & 0.71 & 1 & 1 & 0.75 & 0.72 & 1 & 1 & $<0.5$& 0.75 & 0.72 & 1 & 1 & $<0.5$& 0.75 & \textbf{0.72} & 1 & 1 & 5 \\ 
	heart-statlog-un & 270 & 381 & 2 & 0.86 & 0.78 & 17 & 0.83 & 0.77 & 3 & 7 & 0.88 & 0.81 & 3 & 7 & $<0.5$& 0.87 & 0.86 & 3 & 5 & 1 & 0.87 & \textbf{0.86} & 3 & 5 & 145 \\ 
	hepatitis-un & 155 & 361 & 2 & 0.88 & 0.81 & 16 & 0.88 & 0.82 & 1 & 1 & 0.85 & 0.84 & 1 & 1 & $<0.5$& 0.85 & 0.84 & 1 & 1 & $<0.5$& 0.85 & \textbf{0.84} & 1 & 1 & 191 \\ 
	house-votes-84-un & 435 & 16 & 2 & 0.97 & 0.95 & 15 & 0.96 & 0.95 & 1 & 1 & 0.96 & 0.96 & 1 & 1 & $<0.5$& 0.96 & 0.96 & 1 & 1 & $<0.5$& 0.96 & \textbf{0.96} & 1 & 1 & $<0.5$\\ 
	hungarian-un & 294 & 330 & 2 & 0.85 & 0.78 & 17 & 0.85 & 0.78 & 3 & 7 & 0.77 & 0.76 & 2 & 3 & $<0.5$& 0.82 & 0.81 & 1 & 1 & $<0.5$& 0.82 & \textbf{0.81} & 1 & 1 & 170 \\ 
	irish-un & 500 & 112 & 2 & 0.95 & 0.95 & 16 & 0.96 & 0.96 & 3 & 3 & 0.95 & 0.96 & 3 & 3 & $<0.5$& 0.99 & 0.99 & 2 & 2 & $<0.5$& 1 & \textbf{1} & 4 & 7 & $<0.5$\\ 
	mouse-un & 70 & 45 & 2 & 0.97 & 0.91 & 13 & 0.94 & 0.84 & 3 & 5 & 0.97 & 0.9 & 3 & 5 & $<0.5$& 0.97 & 0.91 & 3 & 3 & $<0.5$& 0.97 & \textbf{0.91} & 3 & 3 & $<0.5$\\ 
	mux6-un & 128 & 6 & 2 & 0.86 & 0.81 & 13 & 0.73 & 0.61 & 4 & 13 & 1 & 1 & 4 & 13 & $<0.5$& 1 & 1 & 3 & 7 & $<0.5$& 1 & \textbf{1} & 3 & 7 & $<0.5$\\ 
	new-throid-un & 215 & 334 & 3 & 0.78 & 0.71 & 18 & 0.76 & 0.7 & 2 & 2 & 0.8 & 0.74 & 4 & 7 & 13 & 0.8 & 0.74 & 4 & 7 & 167 & 0.8 & \textbf{0.74} & 4 & 7 & 186 \\ 
	promoters-un & 106 & 334 & 2 & 0.96 & 0.85 & 16 & 0.91 & 0.75 & 3 & 7 & 0.99 & 0.79 & 3 & 7 & $<0.5$& 0.93 & 0.79 & 3 & 4 & 2 & 0.96 & \textbf{0.83} & 4 & 5 & 345 \\ 
	shuttleM-un & 14500 & 691 & 2 & 0.89 & 0.89 & 2004 & 0.92 & 0.92 & 4 & 9 & 1 & 1 & 4 & 9 & 154 & 1 & 1 & 4 & 4 & 5169 & 1 & \textbf{1} & 4 & 4 & 5592 \\ 
	spect-un & 267 & 22 & 2 & 0.85 & 0.81 & 14 & 0.81 & 0.78 & 1 & 1 & 0.79 & 0.79 & 1 & 1 & $<0.5$& 0.79 & 0.79 & 1 & 1 & $<0.5$& 0.84 & \textbf{0.81} & 4 & 4 & $<0.5$\\ 
	appendicitis-un-r & 106 & 40 & 2 & 0.92 & 0.88 & 15 & 0.93 & 0.88 & 2 & 2 & 0.91 & 0.88 & 1 & 1 & $<0.5$& 0.91 & 0.88 & 1 & 1 & $<0.5$& 0.92 & \textbf{0.9}1 & 3 & 5 & $<0.5$\\ 
	australian-un-r & 690 & 23 & 2 & 0.96 & 0.96 & 16 & 0.97 & 0.97 & 4 & 8 & 0.99 & 0.99 & 4 & 8 & $<0.5$& 0.99 & 0.99 & 3 & 6 & $<0.5$& 0.99 & \textbf{0.99} & 3 & 6 & $<0.5$\\ 
	backache-un-r & 180 & 15 & 2 & 0.96 & 0.94 & 14 & 0.96 & 0.94 & 3 & 5 & 0.95 & 0.97 & 3 & 5 & $<0.5$& 0.98 & 0.97 & 3 & 4 & $<0.5$& 0.98 & \textbf{0.97} & 3 & 4 & $<0.5$\\ 
	cancer-un-r & 449 & 9 & 2 & 0.96 & 0.94 & 15 & 0.92 & 0.9 & 4 & 11 & 0.98 & 0.95 & 4 & 11 & $<0.5$& 0.98 & 0.96 & 4 & 7 & $<0.5$& 0.98 & \textbf{0.96} & 4 & 7 & $<0.5$\\ 
	car-un-r & 1728 & 8 & 2 & 0.9 & 0.9 & 19 & 0.87 & 0.86 & 4 & 8 & 0.97 & 0.97 & 4 & 8 & $<0.5$& 0.97 & 0.97 & 4 & 7 & $<0.5$& 0.97 & \textbf{0.97} & 4 & 7 & $<0.5$\\ 
	cleve-un-r & 302 & 6 & 2 & 0.96 & 0.96 & 15 & 0.92 & 0.92 & 4 & 7 & 1 & 1 & 4 & 7 & $<0.5$& 1 & 1 & 4 & 6 & $<0.5$& 1 & \textbf{1} & 4 & 6 & $<0.5$\\ 
	colic-un-r & 357 & 10 & 2 & 0.96 & 0.95 & 16 & 0.96 & 0.95 & 4 & 8 & 0.99 & 0.99 & 3 & 6 & $<0.5$& 0.99 & 0.99 & 3 & 5 & $<0.5$& 0.99 & \textbf{0.99} & 3 & 5 & $<0.5$\\ 
	corral-un-r & 160 & 6 & 2 & 0.93 & 0.9 & 15 & 0.84 & 0.81 & 4 & 11 & 1 & 1 & 4 & 11 & $<0.5$& 1 & 1 & 4 & 7 & $<0.5$& 1 & \textbf{1} & 4 & 7 & $<0.5$\\ 
	haberman-un-r & 289 & 15 & 2 & 0.96 & 0.94 & 15 & 0.96 & 0.94 & 4 & 8 & 0.98 & 0.97 & 4 & 8 & $<0.5$& 0.98 & 0.97 & 4 & 7 & $<0.5$& 0.98 & \textbf{0.97} & 4 & 7 & $<0.5$\\ 
	heart-statlog-un-r & 270 & 8 & 2 & 0.93 & 0.92 & 15 & 0.9 & 0.89 & 4 & 12 & 0.99 & 0.97 & 4 & 12 & $<0.5$& 0.98 & 0.98 & 4 & 6 & $<0.5$& 0.98 & \textbf{0.98} & 4 & 6 & $<0.5$\\ 
	hepatitis-un-r & 155 & 7 & 2 & 0.97 & 0.97 & 14 & 0.99 & 0.99 & 2 & 3 & 0.97 & 0.97 & 2 & 3 & $<0.5$& 0.99 & 0.99 & 2 & 2 & $<0.5$& 0.99 & \textbf{0.99} & 2 & 2 & $<0.5$\\ 
	hungarian-un-r & 293 & 10 & 2 & 0.98 & 0.96 & 16 & 0.97 & 0.96 & 3 & 5 & 0.98 & 0.96 & 3 & 5 & $<0.5$& 0.98 & 0.98 & 3 & 3 & $<0.5$& 0.98 & \textbf{0.98} & 3 & 3 & $<0.5$\\ 
	irish-un-r & 500 & 112 & 2 & 0.95 & 0.95 & 18 & 0.96 & 0.96 & 3 & 3 & 0.95 & 0.96 & 3 & 3 & $<0.5$& 0.99 & 0.99 & 2 & 2 & $<0.5$& 1 & \textbf{1} & 4 & 7 & $<0.5$\\ 
	mouse-un-r & 70 & 45 & 2 & 0.97 & 0.91 & 15 & 0.94 & 0.84 & 3 & 5 & 0.97 & 0.9 & 3 & 5 & $<0.5$& 0.97 & 0.91 & 3 & 3 & $<0.5$& 0.97 & \textbf{0.91} & 3 & 3 & $<0.5$\\ 
	mux6-un-r & 128 & 6 & 2 & 0.86 & 0.82 & 16 & 0.73 & 0.62 & 4 & 13 & 1 & 1 & 4 & 13 & $<0.5$& 1 & 1 & 3 & 7 & $<0.5$& 1 & \textbf{1} & 3 & 7 & $<0.5$\\ 
	promoters-un-r & 106 & 6 & 2 & 0.95 & 0.91 & 14 & 0.9 & 0.82 & 4 & 9 & 0.99 & 0.92 & 4 & 9 & $<0.5$& 0.97 & 0.92 & 4 & 6 & $<0.5$& 0.97 & \textbf{0.92} & 4 & 6 & $<0.5$\\ 
	shuttleM-un-r & 14500 & 5 & 2 & 0.92 & 0.92 & 45 & 0.9 & 0.9 & 4 & 8 & 1 & 1 & 4 & 8 & $<0.5$& 1 & 1 & 3 & 3 & $<0.5$& 1 & \textbf{1} & 3 & 3 & $<0.5$\\ 
	spect-un-r & 228 & 9 & 2 & 0.98 & 0.98 & 14 & 0.98 & 0.97 & 1 & 1 & 0.97 & 0.97 & 1 & 1 & $<0.5$& 0.97 & 0.97 & 1 & 1 & $<0.5$& 0.97 & \textbf{0.97} & 1 & 1 & $<0.5$\\ 
\end{tabular}
}
\end{table}


==> peter_pseudocode.tex <==
\begin{quote}
\begin{tabbing} xx \= xx \= xx \= xx \= xx \= xx \= xx \= \kill
\textsf{MT}($F, depth, size, UB$) \\
\> \textbf{if}($depth = 0 \vee size = 0 \vee |D(F)^+| = 0 \vee |D(F)^-| =
0$) \\
\> \> \textbf{return} $\textsc{Class}( |D(F)^+| > |D(F)^-| ? pos : neg )$ \\
\> \textbf{if} ($ct = cache[F,depth,size] \neq \bot$) %\\
%\> \> 
\textbf{return} $ct$ \\
\> \textbf{if} ($lb = \textsf{get\_lb}(F,depth,size) > UB$) \\
\> \> \textbf{return} $\textsc{Lb}(lb)$ \\
\> \textbf{if} ($depth = 2$) \\
\> \> $t = \textsf{depth2}(F,size)$ \\
\> \> \textbf{foreach}$(s \in size(t)..size)$ \\
\> \> \> $cache[F,2,s] = t$ \\
\> \> \textbf{return} $t$ \\
\> $bt = \bot$ \% $score(\bot) = \infty$  \\
\> $max\_size = min(2^{depth-1}-1,size-1)$ \\
\> $min\_size = size - max\_size - 1$ \\
\> \textbf{foreach}($f \in \mathcal{F}, f \not\in F, \overline{f} \not\in F$) \\
\> \> \textbf{foreach}$(sl \in min\_size .. max\_size)$ \\
\> \> \> $lt = \textsf{MT}(F \cup \{\overline{f}\}, depth-1, sl, UB)$ \\
\> \> \> \textbf{if} ($score(lt) > UB$) \\
\> \> \> \> $olb = score(lt) + \textsf{get\_lb}(F\cup \{f\},depth-1,size-1-sl)$ \\
\> \> \> \> \textbf{if}($olb < score(bt)$) $bt = \textsc{Lb}(olb)$ \\ 
\> \> \> \> \textbf{continue} \\
\> \> \> $sr = size - size(lt) - 1$ \\
\> \> \> $rt = \textsf{MT}(F \cup \{f\}, depth-1,sr, UB-score(lt))$ \\
\> \> \> \textbf{if}($rt \equiv \textsc{Lb}(\_) \vee lt \equiv \textsc{Lb}(\_)$) % \\
%\> \> \> \> 
$t = \textsc{Lb}(score(lt) + score(rt))$ \\
\> \> \> \textbf{else} $t = \textsc{Decision}(f,lt,rt)$ \\ 
\> \> \> \textbf{if}($score(t) < score(bt)$) $bt = t$ \\
\> \> \> $UB = min(UB,score(t)-1)$ \\
\> \textbf{if} ($bt \equiv \textsc{Lb}(\_))$ \\
\> \> $cache[F,depth,size] = bt$ \\
\> \textbf{else} \\
\> \> \textbf{foreach}$(s \in size(bt)..size)$ \\
\> \> \> $cache[F,depth,s] = bt$ \\
\> \textbf{return} $bt$ \\
\end{tabbing}
\end{quote}


\begin{quote}
\begin{tabbing} xx \= xx \= xx \= xx \= xx \= xx \= xx \= \kill
\textsf{get\_lb}($F, depth, size$) \\
\> $ct = cache[F,depth,size]$ \\
\> $lb = score(ct)$ \\
\> $s = size+1$ \\
\> \textbf{while}($s \leq SIZEBOUND \wedge lb = \infty$) \\
\> \> $lb = score(cache[F,depth,s])$ \\
\> \> $s = s + 1$ \\ 
\> \textbf{if} ($lb = \infty$) $lb = 0$ \\
\> \textbf{foreach}($F'$ close to $F$ where $cache[F',depth,size] \neq \bot$) \\
\> \> \textbf{if} ($LB(D(F),D(F'),depth,size) > lb$) \\
\> \> \> $lb = LB(D(F),D(F'),depth,size)$ \\
\> \textbf{if} ($ct = \bot \vee ct \equiv \textsc{Lb})\_)$) \\
\> \> $cache[F,Depth,size] = \textsc{Lb}(lb)$ \\
\> \textbf{return} $lb$ \\
\end{tabbing}
\end{quote}

==> table_part_three.tex <==
\begin{table}
\caption{Comparison of our default approach (dynamic post-order node selection and in-order feature selection) with a fixed post-order strategy and a feature selection strategy in decreasing Gini coefficients. For each dataset, the number of instances ($\mathcal{D}$), number of binary features ($\mathcal{F}$), and number of classes ($\mathcal{C}$) are displayed. Entries display runtime in seconds (rounded to nearest integer) to compute the optimal classification tree of depth four. Datasets solved under a second or when the differences between the variants was negligible have been omitted.\label{table:partthree} \emir{to be updated} }%
\centering
\resizebox{0.75\columnwidth}{!}{
\def\d{@{\hspace*{1.7mm}}}
\begin{tabular}{ \d l | r | r | r | r r r \d }
	Name &  $|\mathcal{D}|$ & $|\mathcal{F}|$ & $|\mathcal{C}|$ & PostOrder & Gini & Default \\ \hline
	anneal & 812 & 93 & 2 & 1 & 1 & $\bm{<}\textbf{0.5}$ \\ 
	audiology & 216 & 148 & 2 & \textbf{1} & \textbf{1} & \textbf{1} \\ 
	australian-credit & 653 & 125 & 2 & \textbf{2} & 4 & \textbf{2} \\ 
	breast-wisconsin & 683 & 120 & 2 & \textbf{1} & 2 & \textbf{1} \\ 
	diabetes & 768 & 112 & 2 & \textbf{3} & 4 & \textbf{3} \\ 
	german-credit & 1000 & 112 & 2 & \textbf{3} & 4 & \textbf{3} \\ 
	heart-cleveland & 296 & 95 & 2 & \textbf{1} & \textbf{1} & \textbf{1} \\ 
	hypothyroid & 3247 & 88 & 2 & \textbf{2} & 3 & \textbf{2} \\ 
	ionosphere & 351 & 445 & 2 & 149 & 251 & \textbf{101} \\ 
	kr-vs-kp & 3196 & 73 & 2 & 2 & 2 & \textbf{1} \\ 
	letter & 20000 & 224 & 2 & 459 & 603 & \textbf{333} \\ 
	mushroom & 8124 & 119 & 2 & \textbf{1} & $\bm{<}\textbf{0.5}$ & \textbf{1} \\ 
	pendigits & 7494 & 216 & 2 & 96 & 177 & \textbf{95} \\ 
	splice-1 & 3190 & 287 & 2 & 167 & 112 & \textbf{163} \\ 
	vehicle & 846 & 252 & 2 & 19 & 30 & \textbf{12} \\ 
	yeast & 1484 & 89 & 2 & \textbf{2} & 3 & \textbf{2} \\ 
	biodeg & 1055 & 81 & 2 & \textbf{1} & 2 & \textbf{1} \\ 
	default\_credit & 30000 & 44 & 4 & 9 & 9 & \textbf{7} \\ 
	HTRU\_2 & 17898 & 57 & 2 & \textbf{3} & 4 & \textbf{3} \\ 
	Ionosphere & 351 & 143 & 2 & \textbf{2} & \textbf{2} & \textbf{2} \\ 
	magic04 & 19020 & 79 & 2 & 7 & 10 & \textbf{6} \\ 
	spambase & 4601 & 132 & 2 & 17 & 13 & \textbf{11} \\ 
	Statlog\_satellite & 4435 & 385 & 6 & 294 & \textbf{209} & 276 \\ 
	Statlog\_shuttle & 43500 & 181 & 7 & \textbf{60} & 124 & 63 \\ 
	appendicitis-un & 106 & 530 & 2 & \textbf{9} & 35 & \textbf{9} \\ 
	australian-un & 690 & 1163 & 2 & 556 & 639 & \textbf{530} \\ 
	backache-un & 180 & 475 & 2 & \textbf{11} & 18 & 12 \\ 
	cancer-un & 683 & 89 & 2 & $\bm{<}\textbf{0.5}$ & 1 & $\bm{<}\textbf{0.5}$ \\ 
	cleve-un & 303 & 395 & 2 & 11 & 15 & \textbf{10} \\ 
	colic-un & 368 & 415 & 2 & 23 & 33 & \textbf{22} \\ 
	heart-statlog-un & 270 & 381 & 2 & \textbf{8} & 15 & \textbf{8} \\ 
	hepatitis-un & 155 & 361 & 2 & 7 & 12 & \textbf{6} \\ 
	hungarian-un & 294 & 330 & 2 & 7 & 11 & \textbf{6} \\ 
	new-throid-un & 215 & 334 & 3 & 14 & 16 & \textbf{13} \\ 
	promoters-un & 106 & 334 & 2 & 2 & $\bm{<}\textbf{0.5}$ & 2 \\ 
	shuttleM-un & 14500 & 691 & 2 & 197 & 386 & \textbf{169} \\ 
\end{tabular}
}
\end{table}

